Efficient, Dynamic Multi-tenant Edge Computation in EdgeOS

In the future, computing will be immersed in the world around us -- from augmented reality to autonomous vehicles to the Internet of Things. Many of these smart devices will offer services that respond in real time to their physical surroundings, requiring complex processing with strict performance guarantees. Edge clouds promise a pervasive computational infrastructure a short network hop away from end devices, but today's operating systems are a poor fit to meet the goals of scalable isolation, dense multi-tenancy, and predictable performance required by these emerging applications. In this paper we present EdgeOS, a micro-kernel based operating system that meets these goals by blending recent advances in real-time systems and network function virtualization. EdgeOS introduces a Featherweight Process model that offers lightweight isolation and supports extreme scalability even under high churn. Our architecture provides efficient communication mechanisms, and low-overhead per-client isolation. To achieve high performance networking, EdgeOS employs kernel bypass paired with the isolation properties of Featherweight Processes. We have evaluated our EdgeOS prototype for running high scale network middleboxes using the Click software router and endpoint applications using memcached. EdgeOS reduces startup latency by 170X compared to Linux processes and over five orders of magnitude compared to containers, while providing three orders of magnitude latency improvement when running 300 to 1000 edge-cloud memcached instances on one server.

==> Makefile <==
NAME=ms
PAPER=$(NAME).tex

default: setupsty quick clean

quick:
	-pdflatex \\nonstopmode\\input $(PAPER)

all: setupsty thorough cleansty

thorough:
	-pdflatex \\nonstopmode\\input $(PAPER)
	bibtex $(NAME)
	pdflatex \\nonstopmode\\input $(PAPER)
	pdflatex \\nonstopmode\\input $(PAPER)

prepress: all
	gs -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dEmbedAllFonts=true -sOutputFile=final.pdf -f $(NAME).pdf

final: prepress

setupsty:
	cp style/* .

cleansty:
	rm -f *.sty *.bst *.cls

clean: cleansty
	rm -f *.aux *.bbl *log *.blg $(NAME).out


==> sections/extra.tex <==

\subsection{From Design: Communication}
\note{Move to implementation?}

%%% MOVE TO IMPLEMENTATION
\eos\ makes the observation that these ring buffers also track the {\em liveness} of memory: messages that have been transmitted are available for reuse.
Each I/O memory region sizes its DMA ring buffers so that they can hold {\em every} message, thus all messages are tracked in these structures, and I/O memory avoids all additional memory allocation data-structures.
Note that the memory overhead for this approach is relatively small:  a word of memory for each message.
If messages are sized to an MTU (1500B) on a 64 bit architecture, the memory tracking overhead is 4\% (= 64/1500).

When {\tt eos\_recv} attempts to receive data from an ingress ring buffer, it will also move already transmitted packets into the ingress ring for future messages.
This integration of transfer of messages into and out of an I/O memory region with the memory management of messages simplifies memory management, and avoids pointer-based structures (aside from the ring itself), thus increasing the integrity of \fwp s that share an I/O memory region.
Additionally, this significantly simplifies concurrent access to the ring buffers.

Transfers between \fwp s that share an I/O memory region are also performed using ring buffers, but as messages are passed by reference, a single ring is used only to transmit and receive the packets.
All such ring buffers are allocated in memory separate from the I/O memory region so that their access permissions are decoupled from that of the I/O memory region itself.
Note that when communicating \fwp s execute on the same core, optimized IPC can be used if they share the same I/O memory, and the message can be passed by reference directly in registers.
%%% MOVE TO IMPLEMENTATION




\head{Inter-\fwp communication end-points.}
The {eos\_send} and {\eos\_recv} APIs operate on specific communication end-points.
Each end-point is an abstraction around
\begin{inparaenum}[(1)]
\item the ring buffers used for communication which may be connected directly to the paired \fwp, or to the \mma\ which forwards it (likely after copying it) to the paired \fwp, and
\item the capabilities that reference kernel end-points when they are used for event notification (\eg\ for synchronous IPC between \fwp s on the same core).
\end{inparaenum}

\head{DPDK Integration.}
DPDK has an asymmetric relationship with each \fwp: they rely on it to properly handle packet memory, while DPDK should not be beholden to \fwp\ behavior.
Thus, as in the asymmetric analysis above, DPDK is given access to the I/O memory regions of each \fwp.
When packets are received, they are demultiplexed through a \note{[Add name of networking data-structure here]}, which identifies the receiving I/O memory region and \fwp.
The \mma\ is then used to {\em copy} the packet into that \fwp 's I/O memory.
When a \fwp\ wishes to transfer a packet onto the wire, DPDK -- with direct access to the I/O memory -- can avoid a copy, and instead directly transfer from the upstream's I/O region.
Though copies on the network path are anathema for traditional high-throughput network processing systems, the \mma\ is asynchronous.
The MMA's throughput is higher than line rate, thus does not impact system throughput.

% liskov, distributed coordination 93 (``replace local computation, with communication'')

\subsection{From Design: control plane}
\note{Move to implementation?}

\head{DPDK integration.}
The activation of \fwp-chains in our current \eos\ prototype is driven by the reception of packets, thus this operation must be integrated with DPDK network packet reception.
The \fwp-chain cache is shared between the \fwp\ manager, and the DPDK reception path, and when DPDK demultiplexes an incoming packet, and finds that a \fwp-chain for it doesn't already exist, it removes and activates a corresponding instance from the cache.
Though we focus here on the DPDK activation of \fwp-chains, the mechanisms are general, and could be integrated with privileged \fwp s for programmatic \fwp-chain activation.

% iec61508 do-178c iso26262, all apps of HC, or spatial + temporal isolation (robs talk in MC section)

%% \head{HW demux - put in related work??}
%% Hardware-based early demultiplexing~\cite{earlydemux} of networking packets to processes has enabled isolated, high-performance library-based~\cite{engler95exokernel} system services~\cite{arakis,etc}, and is further enabled by research toward expanding NIC functionality to perform that demultiplexing with higher fidelity~\cite{asplos16peterNIC}.
%% While this avoids the use of shared memory pools, it relies on network hardware support for multiple queues to isolate principals.
%% Such support is limited, e.g., the common Intel 82599 chipset for 10Gbps NICs only supports up to 128 queues~\cite{noauthor_82599-10-gbe-controller-brief.pdf_nodate}. \note{cut or move to related work?}
% https://www.intel.com/content/dam/www/public/us/en/documents/product-briefs/82599-10-gbe-controller-brief.pdf

\head{Design - Control plane stuff}


\head{\fwp\ checkpoint cache.}
%% \note{Need to make argument that many different tenants/users/principles will execute the same \fwp s, but need distinct instances of them, so this lets us use a cache}
As new flows arrive, they are paired with corresponding \fwp-chains.
The mapping of flows to the logic that should process them changes at relatively slow rate (\eg\ as defined by a SDN controller), thus it makes sense to {\em cache} these computations for future flows.
In contrast to traditional means of creating processes which involves retrieving programs from disk, interpreting the object format, loading them into memory, and often dynamically linking in shared libraries, \eos\ optimizes for the repetitive creation of isolated computations for tenants.
Correspondingly, the Manager creates \fwp-chains from a {\em \fwp-chain cache} that caches entire chains of \fwp s, their interconnections, and their I/O memory.
Starting a \fwp\ chain in response to the arrival of a new tenant requires identifying the corresponding \fwp-chain, and queuing a prepared, cached \fwp-chain instance.

\smhead{Post-initialization checkpoint.}
An important question is what state should each \fwp\ be in within the cache.
Though the most straightforward approach caches \fwp s that are essentially ``fresh'' (with the instruction pointer set to start executing in {\tt main}), we observe that some \fwp s have significant initialization overheads.
For example, we utilize the Click modular router~\cite{morris99click} to provide low-level network function \fwp s.
The initialization of Click takes a configuration which it parses, and creates a collection of {\em elements} that provide the desired functionality.
Thus, we utilize the {\tt eos\_postinit()} API to allow \fwp s to first initialize, then to take a checkpoint that defines the state of \fwp s in the \fwp-chain cache.

\smhead{\fwp-chain termination and reuse.}
When a \fwp\ chain terminates, the Manager {\em reuses} the chain by integrating it back into the \fwp-chain cache.
In doing so, \eos\ must guarantee that the memory of the cached computation represents the checkpointed, post-initialization state.
As this places data-structures into a known and safe state, it ensures the integrity of future \fwp-chain instances.
I/O memory regions and heap memory are sanitized so that message data in past \fwp-chain instances are not visible to future instances, which maintains confidentiality across \fwp-chain instances.

Note that in existing systems, it is common for the {\em restore} operations to involve file system operations, memory management and initialization, page-table and other kernel data-structure management, and execution initialization~\cite{dragovic03xen,criu}.
Termination effectively undoes quite a bit of the work done on restore by deallocating data-structures and memory.
The effective reuse of the structure of \fwp-chains focuses on avoiding this redundant work, and ideally incurs overhead approaches the cost of {\tt memcpy} and {\tt memset} for simply reinitializing the \fwp-chain's memory.
It should be noted that the simple API of \eos\ avoids the dynamic creation of globally referenced resources -- as the underlying capability-based system avoids ambient authority, thus re-initializing \fwp-chains does not have to consider the tracking and removing access to \fwp\ access to resources in global namespaces.

